Enhancing Constraint Programming via Supervised Learning for Job Shop Scheduling

Constraint programming (CP) is a powerful technique for solving constraint satisfaction and optimization problems. In CP solvers, the variable ordering strategy used to select which variable to explore first in the solving process has a significant impact on solver effectiveness. To address this issue, we propose a novel variable ordering strategy based on supervised learning, which we evaluate in the context of job shop scheduling problems. Our learning-based methods predict the optimal solution of a problem instance and use the predicted solution to order variables for CP solvers. \added[]{Unlike traditional variable ordering methods, our methods can learn from the characteristics of each problem instance and customize the variable ordering strategy accordingly, leading to improved solver performance.} Our experiments demonstrate that training machine learning models is highly efficient and can achieve high accuracy. Furthermore, our learned variable ordering methods perform competitively when compared to four existing methods. Finally, we demonstrate that hybridising the machine learning-based variable ordering methods with traditional domain-based methods is beneficial.

==> 05-related_work.tex <==
\section{Related Work}\label{sec::related_work}

\subsection{Methods for tackling job shop scheduling}
\label{sec:methodsjss}

Since the JSS problem is NP-hard, finding optimal or high quality solutions by conventional optimization algorithms still remains a challenge \cite{pinedo_scheduling:_2008}. Hence, a number of  optimization approaches have been proposed to tackle JSS. Commercial optimization solvers, such as CPLEX,  have made significant advances in recent years, though solving large problem instances for JSS is not straightforward and scalability still proves to be a challenge. \citet{KU2016165} investigated the performance of four different mixed integer programming models for the JSS, and they found that good results for moderate sized problems can be achieved via a disjunctive model. Additionally, meta-heuristics have been an active area of research in JSS, where these methods are often able to find near-optimal solutions \cite{LI201693,Kreipl00,jensen_2003}. These methods have drawbacks due to a ``combinatorial explosion'', where for large instances, there is an exponential growth in the solution space. This makes it computationally challenging to navigate the search space (locally or globally) efficiently to determine high-quality solutions. Furthermore, due to the inherent nature of meta-heuristics, problem-domain knowledge (e.g. solution neighbourhood structure, schedule construction heuristics, etc.) is necessary to efficiently design an application specific algorithm. This is a difficult process often requiring a significant amount of trial-and-error.

% , and any changes to the problem (e.g. change in constraints or objectives) can require major changes to the meta-heuristic in order for it to still be effective.

In recent years, CP has been an effective method for solving satisfaction and optimization problems \cite{apt_2003}. There are a number of problem domains where CP is proven to be effective, and scheduling is one of these  \cite{baptiste2012constraint,barreiro2012europa,grimes2010job,Thiruvady2012}. Moreover, CP has also been shown to be effective on JSS. The studies by \citet{beck2011combining} and \citet{watson2008hybrid}, investigated a CP and tabu search hybrid. Their results showed that this hybrid can generate solutions with low variability and are competitive with local search approaches. \citet{grimes2010job} investigated JSS with setup times, and they showed that enhancing the search component of CP can prove to be very effective for this problem. 



\subsection{Machine learning for job shop scheduling and combinatorial optimization problems}
\label{sec:mlcombinatorialoptimization}

ML for combinatorial optimization (MLCO) is not a new idea and different approaches have been proposed in the literature \cite{lodi2017learning,bengio2018machine,mazyavkina2021reinforcement,talbi2021machine}. In their survey, \citet{bengio2018machine} have classified MLCO studies into three categories depending on the role of ML: (1) \textit{end-to-end learning} in which ML is used to directly produce solutions for CO problem instances, (2) \textit{learning to configure algorithm} in which ML is used to efficiently parameterise optimization algorithms (in a broad sense), (3) \textit{ML alongside optimization algorithms} in which ML is used to assist low-level decisions within optimization algorithms. In the operations research and computational intelligence community, MLCO has been investigated extensively and referred to as hyper-heuristics \cite{burke_hyper-heuristics:_2013}. Different from traditional search algorithms that attempt to find good solutions in the solution search space, hyper-heuristics emphasise on exploring the heuristic (or algorithm) search space to find a good way to solve problem instances. Hyper-heuristics can be used for \textit{heuristic generation} or \textit{heuristic selection}. In heuristic generation, hyper-heuristics use a search algorithm (e.g. GP) to generate/discover effective heuristics for a problem subset. Generated heuristics can be used to construct solutions or refine/improve a solution (similar to the above mentioned categories 1 and 2 in \citet{bengio2018machine}). When used for heuristic selection, the goal of hyper-heuristics is to adaptively select low-level heuristics in optimization algorithms to solve problem instances (similar to category 3 in \cite{bengio2018machine}). To avoid confusion, we will use \citet{bengio2018machine}'s categorisation to discuss related work.

Many earlier studies in the MLCO literature examine the methods for \textit{end-to-end learning}. For examples, popular ML algorithms such as decision tree \cite{olafsson_learning_2010}, logistic regression \cite{ingimundardottir_supervised_2011}, artificial neural networks \cite{mouelhi-chibani_training_2010} can be applied to learn constructive heuristics for production scheduling problems and showed that their learned heuristics outperform existing constructive heuristics in the literature. GP is also a popular learning algorithms in this category and many program representations and advanced search techniques have been proposed to improve the quality of learned heuristics \cite{jakobovic_dynamic_2006,Nguyen2017}. There are several reasons for the popularity of \textit{end-to-end learning}. The main reason is that computational efforts required for training in this case is low and learned model/heuristics can be used to generate good solutions very efficiently. The disadvantage of \textit{end-to-end learning} is that there is no guarantee that solutions produced by these methods are optimal or near-optimal. Empirical results \cite{olafsson_learning_2010,Nguyen2017} showed that there is a gap in solution quality between learned constructive heuristics and optimization algorithms, which is less attractive for problems in which optimal solutions are desirable. Moreover, a meta-algorithm or a heuristic template is usually required to construct solutions, which restrict the applicability of learned heuristics. Apart from production scheduling, \textit{end-to-end learning} is also applied to other CO problems such as NASA's resource-constrained scheduling problem \cite{zhang2000solving}, bin packing \cite{Sim:2015:LLH:2811901.2811903}, graph-based problems \cite{khalil2017learning}, and routing problems \cite{bello17,vanLon2018,yu2019,kool2018attention}. 

% The study by \citet{bello17} proposes a framework for neural combinatorial optimization, i.e. the use of artificial neural networks and reinforcement learning for combinatorial optimization problems. They show that their framework is effective on the travelling salesman problem. 

In the last decade, there has been a growing interest in \textit{learning to configure algorithm}. For example, \citet{khalil2016learning,balcan2018learning} developed innovative ML techniques to learn variable selection methods for mixed integer linear program (MILP) solvers. \citet{he2014learning,furian2021machine} used ML to learn node selection methods for MILP solvers. \citet{shen2021learning} developed an ML-based primal heuristic for MILP solvers. \citet{nguyen2021genetic} investigated the use of GP to learn variable selectors in CP, and they show that this method is effective for JSS considering three different objectives. Our proposed methods belong to this category because the learned variable selectors will configure the search of CP based on characteristics of problem instances.

With the recent boost in computing power, many innovative ML techniques have been developed to enhance optimization algorithms for solving combinatorial optimization problems (i.e. \textit{ML alongside optimization algorithms}). \citet{kruber2017learning} used ML to predict if decomposition is needed to reduce the time to solve MILP instances using features including instance characteristics and decomposition statistics. \citet{Bonami18} used ML to predict if linearisation will be more efficient in solving quadratic programming (QP) problem. \citet{basso2020random} used random sampling and ML to learn what are good decompositions \cite{basso2020random}. \citet{Morabit2020mlcs} developed an ML model to select promising columns for column generation. \citet{sun2019using,lauri2019fine,sun2020generalization} used ML to prune the search space of combinatorial optimization problems. \citet{sun2020boosting} developed ML models to enhance the sampling of a metaheuristic. \added[id=AE,comment={Having the literature review at the end of the paper seems very unusual. I'm OK with this but would expect reviewers to ask for it to be moved earlier.}]{While the  research in this paper fits into this wider effort to use ML to improve combinatorial optimisation, it is to the best of our knowledge the first time that it has been used to improve the labelling strategy in constraint programming for solving constraint optimization problems.}


% ML techniques have been developed to learn variable selection methods \cite{khalil2016learning,balcan2018learning} and node selection methods \cite{he2014learning, furian2021machine} for mixed integer linear program solvers.
% to prune the search space of problem instances \cite{sun2019using,lauri2019fine,sun2020generalization}, to select columns for column generation~\cite{Morabit2020mlcs}, and to generate high-quality feasible solutions efficiently \cite{khalil2017learning,kool2018attention,sun2020boosting,shen2021learning}. 
% \SN{Yuan: can you have a quick look to see if the references here belong to the third category?}

% \cite{song2019learning} Learning Variable Ordering Heuristics for Solving Constraint Satisfaction Problems.
% \cite{nguyen2021genetic} A Genetic Programming Approach for Evolving Variable Selectors in Constraint Programming.
% \cite{gregor2018comparative} A comparative analysis of constraint programming and metaheuristics for job-shop scheduling
% \cite{wattez2020learning} Learning variable ordering heuristics with multi-armed bandits and restarts

% \cite{russell2009learning} Learning heuristics for the superblock instruction scheduling problem 

% \cite{olafsson2010learning} Learning effective new single machine dispatching rules from optimal scheduling data; learn which jobs should be dispatched first from optimally solved problem instances. It did not use constraint programming. 

% \cite{ingimundardottir2011supervised} Supervised learning linear priority dispatch rules for job-shop scheduling; logistic regression. 

% \cite{branke2015automated} Automated design of production scheduling heuristics: A review

% \cite{nguyen2016surrogate} Surrogate-assisted genetic programming with simplified models for automated design of dispatching rules 

% \cite{ingimundardottir2018discovering} Discovering dispatching rules from data using imitation learning: A case study for the job-shop problem 

% \cite{zhang2020evolving} Evolving scheduling heuristics via genetic programming with feature selection in dynamic flexible job-shop scheduling 

% \cite{gao2021automated} Automated Coordination Strategy Design Using Genetic Programming for Dynamic Multipoint Dynamic Aggregation
